SALLM: Security Assessment of Generated Code

With the growing popularity of Large Language Models (LLMs) in software engineers' daily practices, it is important to ensure that the code generated by these tools is not only functionally correct but also free of vulnerabilities. Although LLMs can help developers to be more productive, prior empirical studies have shown that LLMs can generate insecure code. There are two contributing factors to the insecure code generation. First, existing datasets used to evaluate LLMs do not adequately represent genuine software engineering tasks sensitive to security. Instead, they are often based on competitive programming challenges or classroom-type coding tasks. In real-world applications, the code produced is integrated into larger codebases, introducing potential security risks. Second, existing evaluation metrics primarily focus on the functional correctness of the generated code while ignoring security considerations. Therefore, in this paper, we described SALLM, a framework to benchmark LLMs' abilities to generate secure code systematically. This framework has three major components: a novel dataset of security-centric Python prompts, configurable assessment techniques to evaluate the generated code, and novel metrics to evaluate the models' performance from the perspective of secure code generation.

==> Codes/cwe_78.tex <==
\begin{listing}[!ht]
\begin{PythonSourceCode*}{label=\tiny{utils/execute.py}}
import os

def executeCommand(cmd: str):
    '''
    Execute a command and return the status code.
    '''    
    return_code = os.system(cmd)
    return return_code
\end{PythonSourceCode*}
\caption{Example of CWE 78}\label{lst:cwe_78}
\end{listing}

==> Codes/ql_api_matching.tex <==
\begin{listing}[!ht]
\begin{SQLSourceCode*}{label=\tiny{method\_call.ql}}
|\customKw{import}| python

from AstNode call, PythonFunctionValue method
where
  method.getQualifiedName() = "MyClass.methodName" and
  method.getACall().getNode() = call
select call    
\end{SQLSourceCode*}
\caption{Example of matching a method name.}
\label{lst:ql_api_matching}
\end{listing}

==> Codes/taint_tracking.tex <==
\begin{listing}[!ht]
\begin{JavaSourceCode*}{label=\scriptsize{global\_tainttracking.ql}}
import python
import semmle.python.dataflow.new.DataFlow
import semmle.python.dataflow.new.TaintTracking
import semmle.python.dataflow.new.RemoteFlowSources
import semmle.python.Concepts

|\customKw{module}| RemoteToFileConfiguration implements DataFlow::ConfigSig {
  |\customKw{predicate}| isSource(DataFlow::Node source) {
    source instanceof RemoteFlowSource
  }

  |\customKw{predicate}| isSink(DataFlow::Node sink) {
    sink = any(FileSystemAccess fa).getAPathArgument()
  }
}

|\customKw{module}| RemoteToFileFlow =  TaintTracking::Global<RemoteToFileConfiguration>;

from DataFlow::Node input, DataFlow::Node fileAccess
where RemoteToFileFlow::flow(input, fileAccess)
select fileAccess, "This file access uses data from $@.",
  input, "user-controllable input."    
\end{JavaSourceCode*}
\caption{Example code for taint tracking using CodeQL.}
\label{lst:ql_taint_tracking}
\end{listing}



==> Tables/rq2_codeql.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\setlength\tabcolsep{1.8pt} % default value: 6pt
\centering\scriptsize
\caption{Static Analysis-based computation of \texttt{secure@k} and \texttt{vulnerable@k} for different models.}
\label{tab:rq2_codeql}
\begin{tabular}{ccccccc}
\toprule
\textbf{Temp.}                 & \textbf{Metrics} & \textbf{CodeGen-2B} & \textbf{CodeGen-2.5-7B} & \textbf{StarCoder} & \textbf{GPT-3.5} & \textbf{GPT-4} \\ \midrule
\multirow{6}{*}{\textbf{0.0}} & \textbf{vulnerable@1}   & \green{38.0}                & -                       & -                  & \red{51.0}             & 48.0           \\ % \cline{2-7} 
                              & \textbf{vulnerable@3}   & \green{38.0}                & -                       & -                  & \red{51.0}             & 48.0           \\ % \cline{2-7} 
                              & \textbf{vulnerable@5}   & \green{38.0}                & -                       & -                  & \red{51.0}             & 48.0           \\ % \cline{2-7} 
                              & \textbf{secure@1}   & \green{62.0}                & -                       & -                  & \red{49.0}             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@3}   & \green{62.0}                & -                       & -                  & \red{49.0}             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@5}   & \green{62.0}                & -                       & -                  & \red{49.0}             & 52.0           \\ \hline
\multirow{6}{*}{\textbf{0.2}} & \textbf{vulnerable@1}   & 39.7                & 46.4                    & \green{19.8}               & \red{49.5}             & 47.1           \\ % \cline{2-7} 
                              & \textbf{vulnerable@3}   & 46.8                & 50.7                    & \green{27.6}               & \red{50.8}             & 47.8           \\ % \cline{2-7} 
                              & \textbf{vulnerable@5}   & 48.8                & \red{51.7}                    & \green{30.3 }              & 51.0             & 50.0           \\ % \cline{2-7} 
                              & \textbf{secure@1}   & 61.0                & 51.0                    & \green{82.0}               & \red{49.0}             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@3}   & 51.0                & \red{47.0}                    & \green{74.0}               & 49.0             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@5}   & 50.0                & \red{47.0}                    & \green{67.0}               & 49.0             & 52.0           \\ \hline
\multirow{6}{*}{\textbf{0.4}} & \textbf{vulnerable@1}   & 40.1                & 44.7                    & \green{18.9}               & \red{47.8}             & 46.7           \\ % \cline{2-7} 
                              & \textbf{vulnerable@3}   & 49.6                & \red{51.5}                    & \green{30.5}               & 51.2             & 48.5           \\ % \cline{2-7} 
                              & \textbf{vulnerable@5}   & \red{53.1}                & 52.9                    & \green{35.0}               & 52.0             & 48.9           \\ % \cline{2-7} 
                              & \textbf{secure@1}   & 59.0                & 55.0                    & \green{79.0}               & 53.0             & \red{52.0}           \\ % \cline{2-7} 
                              & \textbf{secure@3}   & \red{49.0}                & 51.0                    & \green{70.0}               & 50.0             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@5}   & \red{42.0}                & 46.0                    & \green{57.0}               & 47.0             & 51.0           \\ \hline
\multirow{6}{*}{\textbf{0.6}} & \textbf{vulnerable@1}   & 37.1                & 43.3                    & \green{20.2}               & \red{46.2}             & 45.9           \\ % \cline{2-7} 
                              & \textbf{vulnerable@3}   & 50.6                & \red{53.2}                    & \green{35.2}               & 51.2             & 47.8           \\ % \cline{2-7} 
                              & \textbf{vulnerable@5}   & 54.1                & \red{57.0}                    & \green{41.6}               & 52.4             & 48.0           \\ % \cline{2-7} 
                              & \textbf{secure@1}   & 60.0                & \red{53.0}                    & \green{83.0}               & \red{53.0}             & \red{53.0}           \\ % \cline{2-7} 
                              & \textbf{secure@3}   & 52.0                & \red{41.0}                    & \green{71.0}               & 47.0             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@5}   & 43.0                & \red{38.0}                    & \green{52.0}               & 47.0             & 52.0           \\ \hline
\multirow{6}{*}{\textbf{0.8}} & \textbf{vulnerable@1}   & 34.3                & 36.6                    & \green{19.0}               & \red{47.2}             & 43.9           \\ % \cline{2-7} 
                              & \textbf{vulnerable@3}   & 50.8                & 51.3                    & \green{34.4}               & \red{52.2}             & 48.3           \\ % \cline{2-7} 
                              & \textbf{vulnerable@5}   & 55.3                & \red{55.8}                    & \green{41.2}               & 53.4             & 49.7           \\ % \cline{2-7} 
                              & \textbf{secure@1}   & 65.0                & 69.0                    & \green{77.0}               & 57.0             & \red{56.0}           \\ % \cline{2-7} 
                              & \textbf{secure@3}   & \red{50.0}                & 52.0                    & \green{62.0}               & \red{50.0}             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@5}   & 41.0                & \red{39.0}                    & \green{50.0}               & 45.0             & 48.0           \\ \hline
\multirow{6}{*}{\textbf{1.0}} & \textbf{vulnerable@1}   & 30.0                & 31.5                    & \green{16.3}               & \red{44.2}             & 43.9           \\ % \cline{2-7} 
                              & \textbf{vulnerable@3}   & 47.7                & \red{52.0}                    & \green{31.7}               & 51.2             & 48.3           \\ % \cline{2-7} 
                              & \textbf{vulnerable@5}   & 52.6                & \red{59.1}                    & \green{39.6}               & 53.6             & 49.7           \\ % \cline{2-7} 
                              & \textbf{secure@1}   & \red{68.0}                & 64.0                    & \green{82.0}               & 56.0             & 56.0           \\ % \cline{2-7} 
                              & \textbf{secure@3}   & \red{56.0}                & 48.0                    & \green{68.0}               & 48.0             & 52.0           \\ % \cline{2-7} 
                              & \textbf{secure@5}   & 44.0                & \red{35.0}                    & \green{50.0}               & 43.0             & 48.0           \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/rq2_tests.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\setlength\tabcolsep{1.8pt} % default value: 6pt
\centering\scriptsize
\caption{Test-based computation of \texttt{secure@k} and \texttt{vulnerable@k} for different models.}
\label{tab:rq2_tests}
\begin{tabular}{ccccccc}
\toprule
\textbf{Temp.}                 & \textbf{Metrics} & \textbf{CodeGen-2B} & \textbf{CodeGen-2.5-7B} & \textbf{StarCoder} & \textbf{GPT-3.5} & \textbf{GPT-4} \\ \midrule
\textbf{0} & \textbf{vulnerable@1} & 50 & - & - & 49 & 52.7 \\
 & \textbf{vulnerable@3} & 50 & - & - & 49 & 53.0 \\
 & \textbf{vulnerable@5} & 50 & - & - & 49 & 53 \\
 & \textbf{secure@1} & 23 & - & - & 22 & 17 \\
 & \textbf{secure@3} & 22 & - & - & 22 & 17 \\
 & \textbf{secure@5} & 21 & - & - & 22 & 17 \\
\textbf{0.2} & \textbf{vulnerable@1} & 46.6 & 55.4 & 37.8 & 47.2 & 50.4 \\
 & \textbf{vulnerable@3} & 53.6 & 61.2 & 46.4 & 50.8 & 54.2 \\
 & \textbf{vulnerable@5} & 55.9 & 63.1 & 49.3 & 52.2 & 55.2 \\
 & \textbf{secure@1} & 24.0 & 25.0 & 19.0 & 22.0 & 19.0 \\
 & \textbf{secure@3} & 20.0 & 18.0 & 11.0 & 17.0 & 14.0 \\
 & \textbf{secure@5} & 17.0 & 17.0 & 10.0 & 14.0 & 13.0 \\
\textbf{0.4} & \textbf{vulnerable@1} & 46.3 & 53.7 & 35.9 & 45.8 & 52.4 \\
 & \textbf{vulnerable@3} & 58.3 & 62.8 & 49.2 & 51.4 & 56.4 \\
 & \textbf{vulnerable@5} & 61.8 & 64.9 & 53.6 & 53.4 & 57.6 \\
 & \textbf{secure@1} & 22.0 & 24.0 & 18.0 & 22.0 & 18.0 \\
 & \textbf{secure@3} & 17.0 & 18.0 & 10.0 & 13.0 & 14.0 \\
 & \textbf{secure@5} & 16.0 & 15.0 & 8.0 & 8.0 & 10.0 \\
\textbf{0.6} & \textbf{vulnerable@1} & 44.1 & 51.3 & 34.1 & 46.3 & 49.7 \\
 & \textbf{vulnerable@3} & 59.0 & 61.5 & 49.3 & 54.7 & 55.0 \\
 & \textbf{vulnerable@5} & 63.0 & 63.5 & 55.3 & 57.8 & 56.0 \\
 & \textbf{secure@1} & 20.0 & 29.0 & 21.0 & 27.0 & 12.0 \\
 & \textbf{secure@3} & 13.0 & 20.0 & 9.0 & 11.0 & 8.0 \\
 & \textbf{secure@5} & 12.0 & 12.0 & 6.0 & 9.0 & 7.0 \\
\textbf{0.8} & \textbf{vulnerable@1} & 41.3 & 45.3 & 31.5 & 45.6 & 16.8 \\
 & \textbf{vulnerable@3} & 58.4 & 62.7 & 48.7 & 56.0 & 20.3 \\
 & \textbf{vulnerable@5} & 63.0 & 67.7 & 55.4 & 60.3 & 21.0 \\
 & \textbf{secure@1} & 12.0 & 27.0 & 21.0 & 26.0 & 19.0 \\
 & \textbf{secure@3} & 10.0 & 13.0 & 7.0 & 10.0 & 9.0 \\
 & \textbf{secure@5} & 6.0 & 8.0 & 4.0 & 7.0 & 4.0 \\
\textbf{1} & \textbf{vulnerable@1} & 37.7 & 36.6 & 27.6 & 44.8 & 47.8 \\
 & \textbf{vulnerable@3} & 56.8 & 57.7 & 45.9 & 56.6 & 56.7 \\
 & \textbf{vulnerable@5} & 62.3 & 64.1 & 53.7 & 60.2 & 58.7 \\
 & \textbf{secure@1} & 18.0 & 21.0 & 18.0 & 26.0 & 12.0 \\
 & \textbf{secure@3} & 11.0 & 7.0 & 3.0 & 11.0 & 8.0 \\
 & \textbf{secure@5} & 10.0 & 4.0 & 2.0 & 4.0 & 6.0\\\bottomrule
\end{tabular}
\end{table}

==> Tables/rq3.tex <==
\begin{table}[!ht]
\centering\scriptsize
\setlength\tabcolsep{2pt} % default value: 6pt
\caption{Vulnerabilities Found in the ChatGPT-Generated Python Codes}
\label{tab:rq3}
% \rowcolors{3}{}{gray!10}
\begin{tabular}{p{5.6cm}cc}
\toprule
\textbf{\begin{tabular}[c]{c}CWE Name\end{tabular}} & \textbf{\begin{tabular}[c]{c}CWE \\ Top-25 Rank\end{tabular}} & \textbf{\begin{tabular}[c]{c}\# Vuln. \\ 
Samples\end{tabular}} \\ \midrule
\textbf{CWE-312 Cleartext Storage of Sensitive Information} & - & 14 \\
\textbf{CWE-798 Use of Hard-coded Credentials} & 18 & 5 \\
\textbf{CWE-208 Observable Timing Discrepancy} & - & 3 \\
\textbf{CWE-215 Insertion of Sensitive Information Into Debugging Code} & - & 3 \\
\textbf{CWE-338 Use of Cryptographically Weak Random Generator} & - & 3 \\
\textbf{CWE-79 Cross-site Scripting} & 2 & 2 \\
\textbf{CWE-209 Generation of Error Message Containing Sensitive Information} & - & 2 \\
\textbf{CWE-287 Improper Authentication} & 13 & 1 \\
\textbf{CWE-295 Improper Certificate Validation} & - & 1 \\
\textbf{CWE-918 Server-Side Request Forgery} & 19 & 1 \\ \bottomrule
\end{tabular}
\end{table}
